An indirect search for dark matter with a combined analysis of dwarf spheroidal galaxies from VERITAS

Understanding the nature and identity of dark matter is a key goal in the physics community. In the case that TeV-scale dark matter particles decay or annihilate into standard model particles, very-high-energy (VHE) gamma rays (greater than 100 GeV) will be present in the final state. The Very Energetic Radiation Imaging Telescope Array System (VERITAS) is an imaging atmospheric Cherenkov telescope array that can indirectly detect VHE gamma rays in an energy range of 100 GeV to > 30 TeV. Dwarf spheroidal galaxies (dSphs) are ideal candidates in the search for dark matter due to their high dark matter content, high mass-to-light ratios, and their low gamma-ray fluxes from astrophysical processes. This study uses a legacy data set of 638 hours collected on 17 dSphs, built over 11 years with an observing strategy optimized according to the dark matter content of the targets. The study addresses a broad dark matter particle mass range, extending from 200 GeV to 30 PeV. In the absence of a detection, we set the upper limits on the dark matter velocity-weighted annihilation cross section.

==> dmsearch.tex <==
%\textit{Conor}
%*More sensitive analysis methods and updated characterization of instrument make this paper a significant contribution* 
%Predicted signal, annihilation channels considered. If we want to include a section on UHDM interpretation, brief discussion of PPPC versus HDM input spectrum. Describe folding of input spectrum with IRFs, giving details on averaging over IRFs (provided run-wise? Epoch-wise?).\\

The predicted dark matter flux of a dSph is given by the product of two key terms. One is namely the ``particle physics factor" which is based on theoretical models and is constant for any source of dark matter (dSph, galactic center). The other term is the ``astrophysical factor" or ``J-Factor", as described in Section~\ref{sec:targets}.

The predicted flux from dark matter annihilation is given by

\begin{equation}
\phi_{s}(\Delta\Omega)=\underbrace{\frac{1}{4\pi}\frac{\left<\sigma v\right>}{2M^2_{\chi}}\int^{E_{max}}_{E_{min}}\frac{dN}{dE}dE}_{\Phi_{PP}}\times\underbrace{\int_{\Delta\Omega}\frac{dJ}{d\Omega}d\Omega}_{\text{J-factor}},
\end{equation}
where $\Phi_{PP}$ denotes the ``particle physics factor", $M_{\chi}$ is the dark matter particle mass, $\left< \sigma v \right>$ is the thermally averaged cross-section of the DM particles and  $dN/dE$ is the dark matter annihilation spectrum.

Regarding the dark matter annihilation spectrum, $dN/dE'$, there are two possible models: {\tt PPPC4DMID} \citep{Cirelli_2011} and {\tt HDMSpectra} \citep{Bauer_2021}. Both models provide the final-state photon spectra from a range of annihilation channels, but they are accurate in a different dark matter mass range; i.e., {\tt PPPC4DMID} is available in the mass ranges (5 GeV to 100 TeV) while {\tt HDMSpectra} provides a better characterization in a higher mass range (1 TeV to Planck energy). In this study, we employ {\tt PPPC4DMID} for analyzing masses from 200 GeV to $<$ 100 TeV, and {\tt HDMSpectra} for analyzing masses equal or greater than 100 TeV and up to 30 PeV. We note that they are consistent within the mass range from 1 TeV to 100 TeV \citep{Tak_2022}.

We can now describe the expected number of the dark matter events ($\mathcal{S}$) in terms of the dark matter annihilation flux, the J-Factor, and the VERITAS IRFs

\begin{equation}
\mathcal{S}=\frac{\left<\sigma v \right>T_{obs}}{8\pi m^2_{\chi}} \int_0^{\infty} \int_0^{\infty} \frac{dN}{dE'}J(E')A(E')D(E|E')dE'dE,
\label{equation:expectedEvnts}
\end{equation}
where $T_{obs}$ is the total exposure time, $J(E')$ is the integrated J-factor convolved with the VERITAS energy-dependant PSF, $A(E')$ is the VERITAS effective area, and $D(E|E')$ is the energy distribution matrix. Note that the quantities, $E$ ($E'$) and $\Omega$ ($\Omega'$), are the reconstructed (true) photon energy and solid angle, respectively. 

Due to the constantly changing VERITAS response over time and the wide range of time over which these observations have been taken, a time averaged IRF must be used in this analysis. To do this, each run is categorised by night sky background, zenith angle, and the VERITAS epoch. Each category is then weighted by the total exposure time, and a set of time-averaged IRFs are produced for each dSph dataset.

We obtain a set of nine final state photon spectra, assuming a 100\% branching ratio of dark matter particles in nine different annihilation channels: $e^{+}e^{-}$, $\mu^{+}\mu^{-}$, $\tau^{+}\tau^{-}$, $t\bar{t}$, $b\bar{b}$, $W^{+}W^{-}$, $ZZ$, $\gamma\gamma$, and $\nu_e \bar{\nu}_e$.

==> exp.tex <==
% \section{Proportionality between the exposure time and the upper limit}\label{app:prop}

% As described in Section~\ref{sec:mle}, the upper limit can be obtained by computing $\Delta \log \mathcal{L}$, 

% \begin{equation}
%     \Delta \log \mathcal{L} = \log \left(\frac{\mathcal{L}_0}{\mathcal{L}_1} \right) 
%     = N_{off} \log \frac{\mathcal{B}_0}{\mathcal{B}_1} + \mathcal{S} - (1+\alpha)(\mathcal{B}_0-\mathcal{B}_1) + \sum_{i=1}^{N_{on}}{\log{\frac{\alpha \mathcal{B}_0\,p_{b}(E_i)}{\alpha \mathcal{B}_1\,p_{b}(E_i) + \mathcal{S}\,p_{s}(E_i)}}},
% \end{equation}
% where the subscripts 0 and 1 refer to $\mathcal{S} \equiv 0$ and $\mathcal{S} \neq 0$, respectively, as defined in Equation~\ref{eq:ts}. The expected background $\mathcal{B}_0$ is defined as $\mathcal{B}_0=(N_{on}+N_{off})/(\alpha+1)$ \cite{LiMa}. We expect that $\mathcal{B}_1$ should be equal or similar to $\mathcal{B}_0$ with a very small deviation. Assuming that $\mathcal{B}=\mathcal{B}_0 = \mathcal{B}_1$, the above equation becomes

% \begin{equation}
%     \Delta \log \mathcal{L} =  \mathcal{S} + \sum_{i=1}^{N_{on}}{\log{\frac{\alpha \mathcal{B}\,p_{b,i}}{\alpha \mathcal{B}\,p_{b,i} + \mathcal{S}\,p_{s,i}}}},
% \end{equation}

% For the UL calculation, $\Delta \log \mathcal{L}$ should be 1.35, independent of the exposure time. In other words, for two exposure times, $T_1$ and $T_2$, we can get $\mathcal{S}_{T_1}-\mathcal{S}_{T_2} = \delta$, where
% \begin{equation}
%     \delta = \sum_{i=1}^{N_{on}}{\log{\frac{\alpha \mathcal{B}\,p_{b,i}}{\alpha \mathcal{B}\,p_{b,i} + \mathcal{S}\,p_{s,i}}}} \Bigg|_{T_1} - \sum_{i=1}^{N_{on}}{\log{\frac{\alpha \mathcal{B}\,p_{b,i}}{\alpha \mathcal{B}\,p_{b,i} + \mathcal{S}\,p_{s,i}}}} \Bigg|_{T_2}.
% \end{equation}
% For the absence of dark matter signal ($\alpha\mathcal{B} \gg \mathcal{S}$), this value is negligible, $\delta \approx 0$; i.e., $\mathcal{S}_{T_1} = \mathcal{S}_{T_2} = 1.35$. Therefore, if other terms remain the same in Equation~\ref{equation:expectedEvnts}, one can get $\left<\sigma v \right>_1 T_{obs,1} = \left<\sigma v \right>_2 T_{obs,2}$, or 

% \begin{equation}
%     \frac{\left<\sigma v \right>_1}{\left<\sigma v \right>_2} = \frac{T_{obs,2}}{T_{obs,1}}.
% \end{equation}


% \section{Proportionality between the exposure time and the upper limit}\label{app:prop}

% As described in Section~\ref{sec:mle}, the upper limit can be obtained by computing $\Delta \log \mathcal{L}$, 

% \begin{equation}
%     \Delta \log \mathcal{L} = \log \left(\frac{\mathcal{L}_0}{\mathcal{L}_1} \right) 
%     = N_{off} \log \frac{\mathcal{B}_0}{\mathcal{B}_1} + \mathcal{S} - (1+\alpha)(\mathcal{B}_0-\mathcal{B}_1) + \sum_{i=1}^{N_{on}}{\log{\frac{\alpha \mathcal{B}_0\,p_{b}(E_i)}{\alpha \mathcal{B}_1\,p_{b}(E_i) + \mathcal{S}\,p_{s}(E_i)}}},
% \end{equation}
% where the subscripts 0 and 1 refer to $\mathcal{S} \equiv 0$ and $\mathcal{S} \neq 0$, respectively, as defined in Equation~\ref{eq:ts}. The expected background $\mathcal{B}_0$ is defined as $\mathcal{B}_0=(N_{on}+N_{off})/(\alpha+1)$ \cite{LiMa}. We expect that $\mathcal{B}_1$ should be equal or similar to $\mathcal{B}_0$ with a very small deviation. Assuming that $\mathcal{B}=\mathcal{B}_0 = \mathcal{B}_1$, the above equation becomes

% \begin{equation}
%     \Delta \log \mathcal{L} = \mathcal{\mathcal{S}} -\sum_{i=1}^{N_{on}}\log{\left(1+\frac{\mathcal{S}}{\alpha\mathcal{B}}\frac{p_{s,i}}{p_{b,i}}\right)},
% \end{equation}
% If $\mathcal{S} p_{s,i} \ll \alpha\mathcal{B}p_{b,i}$, the logarithm term can be described with the Taylor expansion,
% \begin{equation}
%     \Delta \log \mathcal{L} \simeq  \left(1 -\sum_{i=1}^{N_{on}}\frac{1}{\alpha\mathcal{B}}\frac{p_{s,i}}{p_{b,i}}\right)\mathcal{S}+\sum_{i=1}^{N_{on}}\frac{1}{2}\left(\frac{\mathcal{S}}{\alpha\mathcal{B}}\frac{p_{s,i}}{p_{b,i}}\right)^2+...
% \end{equation}
% When the signal and background spectral distributions are similar ($p_{s,i} \simeq p_{b,i}$) without a strong signal ($N_{on} \simeq \alpha\mathcal{B}$), the second-order term of the expansion becomes important,
% \begin{equation}
%     \Delta \log \mathcal{L} \simeq  \cancelto{\Scale[0.8]{0}}{\left(1 -\frac{N_{on}}{\alpha\mathcal{B}}\right)}\mathcal{S}+\frac{1}{2}\cancelto{\Scale[0.8]{\propto 1/T}}{\frac{N_{on}}{(\alpha\mathcal{B})^2}}\mathcal{S}^2\propto \frac{S^2}{T} \rightarrow \left<\sigma v \right>_{\Scale[0.5]{\rm UL}} \propto 1/\sqrt{T}.
% \end{equation}
% However, when the two distributions are highly distinct (e.g., the DM spectrum), the first-order term can dominate
% \begin{equation}
%     \Delta \log \mathcal{L} \propto \mathcal{S} \propto \left<\sigma v \right>_{\Scale[0.5]{\rm UL}}T  \,\,\,\rightarrow \,\,\,\left<\sigma v \right>_{\Scale[0.5]{\rm UL}}\propto 1/T.
% \end{equation}
